PASHA: Efficient HPO and NAS with Progressive Resource Allocation

Hyperparameter optimization (HPO) and neural architecture search (NAS) are methods of choice to obtain the best-in-class machine learning models, but in practice they can be costly to run. When models are trained on large datasets, tuning them with HPO or NAS rapidly becomes prohibitively expensive for practitioners, even when efficient multi-fidelity methods are employed. We propose an approach to tackle the challenge of tuning machine learning models trained on large datasets with limited computational resources. Our approach, named PASHA, extends ASHA and is able to dynamically allocate maximum resources for the tuning procedure depending on the need. The experimental comparison shows that PASHA identifies well-performing hyperparameter configurations and architectures while consuming significantly fewer computational resources than ASHA.

==> arXiv v2 PASHA/conclusions.tex <==
In this work we have introduced a new variant of Successive Halving called PASHA.
Despite its simplicity, PASHA leads to strong improvements in the tuning time. For example, in many cases it reduces the time needed to about one third compared to ASHA without a noticeable impact on the quality of the found configuration. 
For benchmarks with a small number of rungs (LCBench), PASHA provides more modest speedups but this limitation can be mitigated in practice by adopting a more granular unit of measure for resources. Further work could investigate the definition of rungs and resource levels, with the aim of understanding how they impact the decisions of the algorithm. More broadly this applies not only to PASHA but also to multi-fidelity algorithms in general.

PASHA can also be successfully combined with more advanced search strategies based on Bayesian Optimization to obtain improvements in accuracy at a fraction of the time. In the future, we would like to test combinations of PASHA with transfer-learning techniques for multi-fidelity such as RUSH~\citep{rush} to
further decrease the tuning time.


==> arXiv v2 PASHA/discussion.tex <==
PASHA is designed to speed up finding the best configuration, making HPO and NAS more accessible. To do so, PASHA interrupts the tuning process when it considers the ranking of configurations to be sufficiently stable, not spending
resources on evaluating configurations in later rungs.
However, the benefits of such mechanism will be small in some circumstances. When
the number of rungs is small, there will be few opportunities for PASHA
to interrupt the tuning and provide large speedups. This phenomenon is demonstrated
in Appendix~\ref{app:lcbench} on the LCBench benchmark \citep{Zimmer2021Auto-PyTorchAutoDL}.

Public benchmarks usually fix the minimum resources to one epoch, while the maximum is benchmark-dependent (e.g. 200 epochs for NASBench201 and 50 for LCBench), leaving little control for algorithms like
PASHA in some cases. Appendix~\ref{app:shorttime} analyses the impact of these choices.

For practical usage, we recommend having a maximum amount of resources at least
100 times larger than the minimum amount of resources when using $\eta=3$
(default). This can be achieved by measuring resources with higher granularity 
(e.g. in terms of gradient updates) if needed.

==> arXiv v2 PASHA/experiments.tex <==
In this section we empirically evaluate the performance of PASHA.
Its goal is not to provide a model with a higher accuracy, but to identify the best configuration in a shorter amount of time so that we can then re-train the model from scratch. Overall, we target a significantly faster tuning time and on-par predictive performance when comparing with the models identified by state-of-the-art optimizers like ASHA. Re-training after HPO or NAS is important because HPO and NAS in general require to reserve a significant part of the data (often around 20 or 30\%) to be used as a validation set. Training with fewer data is not desirable because in practice it is observed that training a model on the union of training and validation sets provides better results.

We tested our method on two different sets of experiments. The first set evaluates the algorithm on NAS problems and uses NASBench201~\citep{nas201}, while the second set focuses on HPO and was run on two large-scale tasks from PD1 benchmark~\citep{Wang2021Pre-trainedOptimization}. 
\subsection{Setup}
Our experimental setup consists of two phases: 1) run the hyperparameter optimizer until $N=256$ candidate configurations are evaluated; and 2) use the best
configuration identified in the first phase to re-train the model from scratch. For the purpose of these experiments we re-train all the models using only the training set. This avoids introducing an arbitrary choice on the validation set size and allows us to leverage
standard benchmarks such as NASBench201. In real-world applications the model can be trained on both training and validation sets.
All our results report only the time invested in identifying the best configuration since the re-training time is comparable for all optimizers. All results are averaged over multiple repetitions, with the details specified for each set of experiments separately. We use $N=90$-th percentile when calculating the value of $\epsilon$.

We use 4 workers to perform parallel and asynchronous evaluations. The choice of $R$ is sensitive for ASHA as it can make the optimizer consume too many resources and penalize the performance. For a fair comparison, we make $R$ dataset-dependent taking the maximum amount of resources in the considered benchmarks. $r$ is also dataset-dependent and $\eta$, the halving factor, is set to 3 unless otherwise specified. The same values are used for both ASHA and PASHA. Runtime reported is the time spent on HPO (without retraining), including the time for computing validation set performance. 

We compare PASHA with ASHA \citep{li2020asha}, a widely-adopted approach for multi-fidelity HPO, and other relevant baselines. In particular, we consider ``one-epoch baseline'' that trains all configurations for one epoch (the minimum available resources) and then selects the most promising configuration, and ``random baseline'' that randomly selects the configuration without any training. For both one-epoch and random baselines we sample $N=256$ configurations, using the same scheduler and seeds as for PASHA and ASHA. All reported accuracies are after retraining for $R=200$ epochs. In addition, two, three and five-epoch baselines are evaluated in Appendix \ref{app:additional_baselines}.

\subsection{NAS experiments}
For our NAS experiments we leverage the well-known NASBench201~\citep{nas201} benchmark. The task is to identify the network structure providing the best accuracy on three different datasets (CIFAR-10, CIFAR-100 and ImageNet16-120) independently. We use $r=1$ epoch and $R=200$ epochs. 
We repeat the experiments using 5 random seeds for the scheduler and 3 random seeds for NASBench201 (all that are available), resulting in 15 repetitions. Some configurations in NASBench201 do not have all seeds available, so we impute them by averaging over the available seeds.
To measure the predictive performance we report the best accuracy on the combined validation and test set provided by the creators of the benchmark.

The results in Table~\ref{tab:nas201} suggest PASHA consistently leads to strong improvements in runtime, while achieving similar accuracy values as ASHA. The one-epoch baseline has noticeably worse accuracies than ASHA or PASHA, suggesting that PASHA does a good job of deciding when to continue increasing the resources -- it does not stop too early. Random baseline is a lot worse than the one-epoch baseline, so there is value in performing NAS. We also report the maximum resources used to find how early the ranking becomes stable in PASHA. The large variances are caused by stopping HPO at different rung levels for different seeds (e.g. 27 and 81 epochs). Note that the time required to train a model is about 1.3h for CIFAR-10 and CIFAR-100, and about 4.1h for ImageNet16-120, making the total tuning time of PASHA comparable or faster than the training time.

We also ran additional experiments testing PASHA with a reduction factor of $\eta=2$ and $\eta=4$ instead of $\eta=3$, the usage of PASHA as a scheduler in MOBSTER~\citep{Klein2020Model-basedSearch} and alternative ranking functions. These experiments provided similar findings as the above and are described next.

\begin{table}[t]
\caption{NASBench201 results. PASHA leads to large improvements in runtime, while achieving similar accuracy as ASHA.}
  \label{tab:nas201}
\begin{center}
  \resizebox{0.85\linewidth}{!}{\begin{tabular}{llcccc}
    \toprule
Dataset & Approach & Accuracy (\%) & Runtime & Speedup factor & Max resources \\
 \midrule
\multirow{4}{*}{{CIFAR-10}} & ASHA & 93.85 $\pm$ \phantom{0}0.25 & 3.0h $\pm$ 0.6h & 1.0x & 200.0 $\pm$ \phantom{0}0.0 \\
& PASHA & 93.57 $\pm$ \phantom{0}0.75 & 1.3h $\pm$ 0.6h & 2.3x & \phantom{0}36.1 $\pm$ 50.0 \\
& One-epoch baseline & 93.30 $\pm$ \phantom{0}0.61 & 0.3h $\pm$ 0.0h & 8.5x & \phantom{00}1.0 $\pm$ \phantom{0}0.0 \\
& Random baseline & 72.88 $\pm$ 19.20 & 0.0h $\pm$ 0.0h & N/A & \phantom{00}0.0 $\pm$ \phantom{0}0.0 \\
\midrule
\multirow{4}{*}{{CIFAR-100}} & ASHA & 71.69 $\pm$ \phantom{0}1.05 & 3.2h $\pm$ 0.9h & 1.0x & 200.0 $\pm$ \phantom{0}0.0 \\
& PASHA & 71.84 $\pm$ \phantom{0}1.41 & 0.9h $\pm$ 0.4h & 3.4x & \phantom{0}20.5 $\pm$ 48.3 \\
& One-epoch baseline & 65.57 $\pm$ \phantom{0}5.53 & 0.3h $\pm$ 0.0h & 9.2x & \phantom{00}1.0 $\pm$ \phantom{0}0.0 \\
& Random baseline  & 42.83 $\pm$ 18.20 & 0.0h $\pm$ 0.0h & N/A & \phantom{00}0.0 $\pm$ \phantom{0}0.0 \\
\midrule
\multirow{4}{*}{{ImageNet16-120}} & ASHA & 45.63 $\pm$ \phantom{0}0.81 & 8.8h $\pm$ 2.2h & 1.0x & 200.0 $\pm$ \phantom{0}0.0 \\
& PASHA & 45.13 $\pm$ \phantom{0}1.51 & 2.9h $\pm$ 1.7h & 3.1x & \phantom{0}21.3 $\pm$ 48.1 \\
& One-epoch baseline & 41.42 $\pm$ \phantom{0}4.98 & 1.0h $\pm$ 0.0h & 8.8x & \phantom{00}1.0 $\pm$ \phantom{0}0.0 \\
& Random baseline & 20.75 $\pm$ \phantom{0}9.97 & 0.0h $\pm$ 0.0h & N/A & \phantom{00}0.0 $\pm$ \phantom{0}0.0 \\
\bottomrule
\end{tabular}}
\end{center}
\end{table}

\subsubsection{Reduction factor}
An important parameter for the performance of multi-fidelity algorithms like ASHA is the reduction factor. This hyperparameter controls the fraction of pruned candidates at every rung. The optimal theoretical value is $e$ and it is typically set to 2 or 3.
In Table~\ref{tab:reduction_factor} we report the results of the different algorithms ran with $\eta=2$ and $\eta=4$ on CIFAR-100 (the full set of results is in Appendix \ref{app:reduction}). The gains are consistent also for $\eta=2$ and $\eta=4$, with a larger speedup when using $\eta=2$ as that allows PASHA to make more decisions and identify earlier that it can stop the search.
  
\begin{table}[H]
\caption{NASBench201 -- CIFAR-100 results with various reduction factors $\eta$. \revised{The speedup is large for both $\eta=2$ and $\eta=4$, and accuracy similar to ASHA is retained.}}
\label{tab:reduction_factor}
\begin{center}
\resizebox{0.85\linewidth}{!}{\begin{tabular}{lclcccc}
  \toprule
Dataset & Reduction factor & Approach & Accuracy (\%) & Runtime & Speedup factor & Max resources \\
\midrule
\multirow{4}{*}{{CIFAR-100}} & \multirow{2}{*}{{$\eta=2$}} & ASHA & 71.67 $\pm$ 0.84 & \phantom{0}3.8h $\pm$ 1.0h & 1.0x & 200.0 $\pm$ \phantom{0}0.0 \\
& & PASHA & 71.65 $\pm$ 1.42 & \phantom{0}0.9h $\pm$ 0.1h & 4.2x & \phantom{00}5.9 $\pm$ \phantom{0}2.0 \\
& \multirow{2}{*}{{$\eta=4$}} & ASHA & 71.43 $\pm$ 1.13 & \phantom{0}2.7h $\pm$ 0.9h & 1.0x & 200.0 $\pm$ \phantom{0}0.0 \\
& & PASHA & 72.09 $\pm$ 1.22 & \phantom{0}1.0h $\pm$ 0.4h & 2.8x & \phantom{0}25.1 $\pm$ 49.0 \\
\bottomrule
\end{tabular}}
\end{center}
\end{table}

\subsubsection{Bayesian Optimization}
Bayesian Optimization combined with multi-fidelity methods such as Successive Halving can improve the predictive performance of the final model~\citep{Klein2020Model-basedSearch}. In this set of experiments, we verify PASHA can speedup also these kinds of methods.
Our results are reported in Table~\ref{tab:nasbench_BO}, where we can clearly see PASHA obtains a similar accuracy result as ASHA with significant speedup.

\begin{table}[H]
\caption{NASBench201 results for ASHA with Bayesian Optimization searcher -- MOBSTER \citep{Klein2020Model-basedSearch} and similarly extended version of PASHA. The results show PASHA can be successfully combined with a smarter configuration selection strategy.}
\begin{center}
  \resizebox{0.8\linewidth}{!}{\begin{tabular}{llcccc}
    \toprule
Dataset & Approach & Accuracy (\%) & Runtime & Speedup factor & Max resources \\
\midrule
\multirow{2}{*}{CIFAR-10} & MOBSTER & 94.21 $\pm$ 0.28 & \phantom{0}5.0h $\pm$ 1.1h & 1.0x & 200.0 $\pm$ 0.0 \\
& PASHA BO & 94.00 $\pm$ 0.20 & \phantom{0}2.6h $\pm$ 1.8h & 2.0x & \phantom{0}70.7 $\pm$ 81.6 \\
\midrule
\multirow{2}{*}{CIFAR-100} & MOBSTER & 72.79 $\pm$ 0.68 & \phantom{0}5.7h $\pm$ 1.4h & 1.0x & 200.0 $\pm$ 0.0 \\
& PASHA BO & 72.16 $\pm$ 1.07 & \phantom{0}1.6h $\pm$ 0.5h & 3.7x & \phantom{0}13.0 $\pm$ 8.7 \\
\midrule
\multirow{2}{*}{ImageNet16-120} & MOBSTER & 46.21 $\pm$ 0.70 & 15.1h $\pm$ 4.0h & 1.0x & 200.0 $\pm$ 0.0 \\
& PASHA BO & 45.36 $\pm$ 1.06 & \phantom{0}3.9h $\pm$ 1.2h & 3.9x & \phantom{0}11.8 $\pm$ 7.9 \\
\bottomrule
\end{tabular}}
\label{tab:nasbench_BO}
\end{center}
\end{table}

\subsubsection{Alternative ranking functions}
We have considered a variety of alternative ranking functions in addition to the soft ranking function that automatically estimates the value of $\epsilon$ by measuring noise in rankings. These include simple ranking (equivalent to soft ranking with $\epsilon = 0.0$), soft ranking with fixed values of $\epsilon$ or obtained using various heuristics (for example based on the standard deviation of objective values in the previous rung), Rank Biased Overlap (RBO) \citep{webber2010rbo}, and our own reciprocal rank regret metric (RRR) that considers the objective values of configurations. Details of the ranking functions and additional results are in Appendix~\ref{app:ranking}.

Table \ref{tab:cifar100_rank_f_subset} shows a selection of the results on CIFAR-100 with full results in the appendix. We can see there are also other ranking functions that work well and that simple ranking is not sufficiently robust -- some benevolence is needed. However, the ranking function that estimates the value of $\epsilon$ by measuring noise in rankings (to which we refer simply as PASHA) remains the easiest to use, is well-motivated and offers both excellent performance and large speedup.
  \begin{table}[h!]
    \caption{NASBench201 -- CIFAR-100 results for a variety of ranking functions\revised{, showing there are also other well-performing options, even though those are harder to use and are less interpretable.}}
    \label{tab:cifar100_rank_f_subset}
\begin{center}
    \resizebox{0.8\linewidth}{!}{\begin{tabular}{lcccc}
      \toprule
 Approach  & Accuracy (\%) & Runtime (s) & Speedup factor & Max resources \\
  \midrule
ASHA & 71.69 $\pm$ \phantom{0}1.05 & 3.2h $\pm$ 0.9h & 1.0x & 200.0 $\pm$ \phantom{0}0.0 \\
PASHA & 71.84 $\pm$ \phantom{0}1.41 & 0.9h $\pm$ 0.4h & 3.4x & \phantom{0}20.5 $\pm$ 48.3 \\
  \midrule
PASHA direct ranking & 71.69 $\pm$ \phantom{0}1.05 & 2.8h $\pm$ 0.7h & 1.1x & 200.0 $\pm$ \phantom{0}0.0 \\
  \midrule
PASHA soft ranking $\epsilon=2.5\%$ & 71.41 $\pm$ \phantom{0}1.15 & 1.5h $\pm$ 0.7h & 2.1x & \phantom{0}88.3 $\pm$ 74.4 \\
PASHA soft ranking $\epsilon=2\sigma$ & 71.14 $\pm$ \phantom{0}0.97 & 1.9h $\pm$ 0.7h & 1.7x & 136.4 $\pm$ 75.8 \\
  \midrule
PASHA RBO & 71.51 $\pm$ \phantom{0}0.93 & 2.4h $\pm$ 0.7h & 1.3x & 180.5 $\pm$ 50.6 \\
PASHA RRR & 71.42 $\pm$ \phantom{0}1.51 & 1.2h $\pm$ 0.5h & 2.6x & \phantom{0}39.3 $\pm$ 51.4 \\
  \midrule
One-epoch baseline  & 65.57 $\pm$ \phantom{0}5.53 & 0.3h $\pm$ 0.0h & 9.2x & \phantom{00}1.0 $\pm$ \phantom{0}0.0 \\
Random baseline & 42.83 $\pm$ 18.20 & 0.0h $\pm$ 0.0h & N/A & \phantom{00}0.0 $\pm$ \phantom{0}0.0 \\
      \bottomrule
    \end{tabular}}
\end{center}
  \end{table}


\subsection{HPO experiments}
We further utilize the PD1 HPO benchmark \citep{Wang2021Pre-trainedOptimization} to show the usefulness of PASHA in large-scale settings. In particular, we take WMT15 German-English \citep{Bojar2015FindingsTranslation} and ImageNet \citep{Deng2009Imagenet:Database} datasets that use xformer \citep{xFormers2021} and ResNet50 \citep{He2015DeepRecognition} models. Both of them are datasets with a large amount of training examples, in particular WMT15 German-English has about 4.5M examples, while ImageNet has about 1.3M examples.

In PD1 we optimize four hyperparameters: base learning rate $\eta \in \left[10^{-5}, 10.0\right]$ (log scale), momentum $1-\beta \in \left[10^{-3}, 1.0\right]$ (log scale), polynomial learning rate decay schedule power $p \in \left[0.1, 2.0\right]$ (linear scale) and decay steps fraction $\lambda \in \left[0.01, 0.99\right]$ (linear scale). The minibatch size used for WMT experiments is 64, while the minibatch size for ImageNet experiments is 512. There are 1414 epochs available for WMT and 251 for ImageNet. There are also other datasets in PD1, but these only have a small number of epochs with 1 epoch being the minimum amount of resources. As a result there would not be enough rungs to see benefits of the early stopping provided by PASHA. If resources could be defined in terms of fractions of epochs, PASHA could be beneficial there too. Most public benchmarks have resources defined in terms of epochs, but in practice it is possible to define resources also in alternative ways. We use 1-NN as a surrogate model for the PD1 benchmark. We repeat our experiments using 5 random seeds and there is only one dataset seed available.

The results in Table \ref{tab:hpo_experiments_pd1} show that PASHA leads to large speedups on both WMT and ImageNet datasets. The speedup is particularly impressive for the significantly larger WMT dataset where it is about 15.5x, highlighting how PASHA can significantly accelerate the HPO search on datasets with millions of training examples (WMT has about 4.5M training examples). The one-epoch baseline obtains similar accuracy as ASHA and PASHA for WMT, but performs significantly worse on ImageNet dataset. This result suggests that simple approaches such as the one-epoch baseline are not robust and solutions such as PASHA are needed (which we also saw on NASBench201). Selecting the hyperparameters randomly leads to significantly worse performance than any of the other approaches.

\begin{table}[H]
  \caption{Results of the HPO experiments on WMT and ImageNet tasks from the PD1 benchmark. Mean and std of the best validation accuracy (or its equivalent as given in the PD1 benchmark).}
  \label{tab:hpo_experiments_pd1}
\begin{center}
  \resizebox{0.8\linewidth}{!}{
  \begin{tabular}{llcccc}
    \toprule
Dataset & Approach & Accuracy (\%) & Runtime & Speedup factor & Max resources \\
\midrule
\multirow{4}{*}{{WMT}} & ASHA & 62.72 $\pm$ \phantom{0}1.41 & 43.7h $\pm$ 37.2h & \phantom{0}1.0x & 1357.4 $\pm$ 80.4 \\
& PASHA & 62.04 $\pm$ \phantom{0}2.05 & \phantom{0}2.8h $\pm$ \phantom{0}0.6h & 15.5x & \phantom{00}37.8 $\pm$ 21.6 \\
& One-epoch baseline  & 62.36 $\pm$ \phantom{0}1.40 & \phantom{0}0.6h $\pm$ \phantom{0}0.0h & 67.3x & \phantom{000}1.0 $\pm$ \phantom{0}0.0 \\
& Random baseline  & 33.93 $\pm$ 21.96 & \phantom{0}0.0h $\pm$ \phantom{0}0.0h & N/A & \phantom{000}0.0 $\pm$ \phantom{0}0.0 \\
\midrule
\multirow{4}{*}{{ImageNet}} & ASHA & 75.10 $\pm$ \phantom{0}2.03 & \phantom{0}7.3h $\pm$ \phantom{0}1.2h & \phantom{0}1.0x & \phantom{0}251.0 $\pm$ \phantom{0}0.0 \\
& PASHA & 73.37 $\pm$ \phantom{0}2.71 & \phantom{0}3.8h $\pm$ \phantom{0}1.0h & \phantom{0}1.9x & \phantom{00}45.0 $\pm$ 30.1 \\
& One-epoch baseline  & 63.40 $\pm$ \phantom{0}9.91 & \phantom{0}1.1h $\pm$ \phantom{0}0.0h & \phantom{0}6.7x & \phantom{000}1.0 $\pm$ \phantom{0}0.0 \\
& Random baseline  & 36.94 $\pm$ 31.05 & \phantom{0}0.0h $\pm$ \phantom{0}0.0h & N/A & \phantom{000}0.0 $\pm$ \phantom{0}0.0 \\
\bottomrule
\end{tabular}}
\end{center}
\end{table}




==> arXiv v2 PASHA/intro.tex <==
Hyperparameter optimization (HPO) and neural architecture search (NAS) yield state-of-the-art models, but often are a very costly endeavor, especially when working with large datasets and models.
For example, using the results of \citep{sharir2020nlp} we can estimate that evaluating 50 configurations for a 340-million-parameter BERT model \citep{Devlin2019BERT:Understanding} on the 15GB Wikipedia and Book corpora would cost around \$500,000.
To make HPO and NAS more efficient, researchers explored how we can learn from cheaper evaluations (e.g. on a subset of the data) to later allocate more resources only to promising configurations. This created a family of methods often described as multi-fidelity methods. Two well-known algorithms in this family are Successive Halving (SH)~\citep{jamieson2016non, karnin2013almost} and Hyperband (HB)~\citep{hyperband}.

Multi-fidelity methods significantly lower the cost of the tuning. 
\citet{hyperband} reported speedups up to 30x compared to standard Bayesian Optimization (BO) and up to 70x compared to random search.
Unfortunately, the cost of current multi-fidelity methods is still too high for many practitioners, also because of the large datasets used for training the models. As a workaround, they need to design heuristics which can select a set of hyperparameters or an architecture with a cost comparable to training a single configuration, for example, by training the model with multiple configurations for a single epoch and then selecting the best-performing candidate.

On one hand, such heuristics lack robustness and need to be adapted to
the specific use-cases in order to provide good results. On the other hand, 
they build on an extensive amount of practical experience suggesting that 
multi-fidelity methods are often not sufficiently aggressive in 
leveraging early performance measurements and that identifying the best performing set of hyperparameters (or the best architecture) does not require training a model until convergence.
For example, \citet{bornschein2020small} show that it is possible to find the best hyperparameter -- number of channels in ResNet-101 architecture \citep{He2015DeepRecognition} for ImageNet \citep{Deng2009Imagenet:Database} -- using only one tenth of the data. However, it is not known beforehand that one tenth of data is sufficient for the task.
 
Our aim is to design a method that consumes fewer resources than standard multi-fidelity algorithms such as Hyperband \citep{hyperband} or ASHA \citep{li2020asha}, and yet is able to identify configurations that produce models with a similar predictive performance after full retraining from scratch. Models are commonly retrained on a combination of training and validation sets to obtain the best performance after optimizing the hyperparameters. To achieve the speedup, we propose a variant of ASHA, called Progressive ASHA (PASHA), that starts with a small amount of initial maximum resources and gradually increases them as needed.
ASHA in contrast has a fixed amount of maximum resources, which is a hyperparameter defined by the user and is difficult to select.
Our empirical evaluation shows PASHA can save a significant amount of resources while finding similarly well-performing configurations as conventional ASHA, reducing the entry barrier to do HPO and NAS.

To summarize, our contributions are as follows: 1) We introduce a new approach called PASHA that dynamically selects the amount of maximum resources to allocate for HPO or NAS (up to a certain budget), 2) Our empirical evaluation shows the approach significantly speeds up HPO and NAS without sacrificing the performance, and 3) We show the approach can be successfully combined with sample-efficient strategies based on Bayesian Optimization, highlighting the generality of our approach. Our implementation is based on the Syne Tune library \citep{synetune}.


==> arXiv v2 PASHA/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> arXiv v2 PASHA/method.tex <==
PASHA is an extension of ASHA~\citep{li2020asha} inspired by the ``doubling trick''~\citep{riggedcasino}. PASHA targets improvements for hyperparameter tuning on large datasets by hinging on the assumptions made about the crossing points of the learning curves in Section~\ref{sec:setup}. 
The algorithm starts with a small initial amount of resources and progressively increases them if the ranking of the configurations in the top two \textit{rungs} (rounds of promotion) has not stabilized. The ability of our approach to stop early automatically is the key benefit. We illustrate the approach in Figure \ref{fig:pasha_diagram}, showing how we stop evaluating configurations for additional rungs if rankings are stable.

\begin{figure}[ht]
\begin{center}
\includegraphics[width=0.49\linewidth]{images/PASHAEarlyStop.png}
\includegraphics[width=0.49\linewidth]{images/PASHANotEarlyStop.png}
\caption{Illustration of how PASHA stops early if the ranking of configurations has stabilized. Left: the ranking of the configurations (displayed inside the circles) has stabilized, so we can select the best configuration and stop the search. Right: the ranking has not stabilized, so we continue.}
\label{fig:pasha_diagram}
\end{center}
\end{figure}

We describe the details of our proposed approach in Algorithm \ref{alg:pasha}. Given $\eta$, a hyperparameter used both in ASHA and PASHA to control the fraction of configurations to prune, PASHA sets the current maximum resources \revised{$R_t$} to be used for evaluating a configuration using the reduction factor $\eta$ and the minimum amount of resources $r$ to be used \revised{($K_t$ is the current maximum rung)}. The approach increases the maximum number of resources allocated to promising configurations each time the ranking of configurations in the top two rungs becomes inconsistent. For example, if we can currently train configurations up to rung 2 and the ranking of configurations in rung 1 and rung 2 is not consistent, then we allow training part of the configurations up to rung 3, i.e. one additional rung.

The minimum amount of resources $r$ is a hyperparameter to be set by the user. 
It is significantly easier to set compared to $R$ as $r$ is the minimum amount of resources required to see a meaningful difference in the performance of the models, and it can be easily estimated empirically by running a few small-scale experiments.

\begin{algorithm}[h!]
\begin{algorithmic}[1]
\footnotesize
\State \textbf{input} {minimum resource $r$, reduction factor $\eta$} 
\smallskip
\Function{${\small \texttt{PASHA}}()$}{}
\State { \revised{$t=0, R_0 = \eta r$, $K_0=\lfloor\log_\eta(R_0/r)\rfloor$}}
\While{desired}
\For{\upshape each free worker}
\State $(\theta, k) = {\small \texttt{get\_job}}()$
\State ${\small \texttt{run\_then\_return\_val\_loss}}(\theta, r\eta^{k})$ 
\EndFor
\For{\upshape completed job ($\theta$, $k$) with loss $l$} 
\State Update configuration $\theta$ in rung $k$ with loss $l$
\If{ \revised {$k \geq K_t - 1$}}
  \State $\pi_k = \texttt{configuration\_ranking}(k)$
\EndIf
\If{\revised{$k = K_t$} and $\pi_k \not\equiv \pi_{k-1}$} 
  \State $t = t+1$
  \State{$R_t=\eta^t R_0$}
  \State{$K_t=\lfloor\log_\eta(R_t/r)\rfloor$}
\EndIf
\EndFor
\EndWhile
\EndFunction
\smallskip
\Function{${\small \texttt{get\_job}}()$}{}
\State {\small $\texttt{// Check if there is a promotable config}$}
\For{$k=K_t-1,\dots,1,0$} 
\State candidates $={\small \texttt{top\_k}}(\text{rung } k, |\text{rung } k|/\eta)$ 
\State promotable $=\{c \in \text{candidates}:c \text{ not promoted} \}$ 
\If{\upshape $|\text{promotable}|>0$}
\State \textbf{return} \upshape $\text{promotable}[0], k + 1$
\EndIf
\State {\small \texttt{// If not, grow bottom rung}}
\State Draw random configuration $\theta$ 
\State \textbf{return} $\theta, 0$
\EndFor
\EndFunction
\end{algorithmic}
\caption{Progressive Asynchronous Successive Halving (PASHA)}
\label{alg:pasha}
\end{algorithm}

We also set a maximum amount of resources $R$ so that PASHA can default to ASHA if needed and avoid increasing the resources indefinitely. While it is not generally reached, it provides a safety net.

\subsection{Soft ranking}
Due to the noise present in the training process, negligible differences in the measured predictive performance of different configurations can lead to  significantly different rankings. For these reasons we adopt what we call ``soft ranking''.
In soft ranking, configurations are still sorted by predictive performance but are considered equivalent if the performance difference is smaller than a value $\epsilon$ (or equal to it). Instead of producing a sorted list of configuration, this provides a list of lists
where for every position of the ranking there is a list of equivalent configurations. The concept is explained graphically in Figure~\ref{fig:soft_ranking}, and we also provide a formal definition.
For a set of $n$ configurations $c_1, c_2, \cdots, c_i, \cdots, c_n$ and performance metric $f$ (e.g. accuracy) with $f(c_1) \leq f(c_2) \leq \cdots \leq f(c_i) \leq \cdots \leq f(c_n)$, soft rank at position $i$ is defined as
$$\text{soft rank}_i = \left\{c_j \in \text{configurations} : |f(c_i)-f(c_j)|\leq\epsilon \right\}.$$

When deciding on if to increase the resources, we go through the ranked list of configurations in the top rung and check if the current configuration at the given rank was in the list of configurations for that rank in the previous rung. If there is a configuration which does not satisfy the condition, we increase resources. 

\begin{figure}[h!]
\begin{center}
    \includegraphics[width=0.8\textwidth]{images/soft_ranking_curves.png}
    \caption{Illustration of soft ranking. There are three lists with the first two containing two items because the scores of the two configurations are closer to each other than $\epsilon$.}
    \label{fig:soft_ranking}
\end{center}
\end{figure}



\subsection{Automatic estimation of $\epsilon$ by measuring noise in rankings}
Every operation involving randomization gives slightly different results when repeated, the training process and the measurement of performance on the validation set are no exception. 
In an ideal world, we could repeat the process multiple times to compute empirical mean and variance to make a better decision. Unfortunately this is not possible in our case since the repeating portions of the training process will defeat the purpose of our work: speeding up the tuning process. Understanding when the differences between the performance measured for different configurations are ``significant'' is crucial for ranking them correctly. We devise a method to estimate a threshold below which differences are meaningless.

Our intuition is that configurations with different performance maintain their relative ranking over time. On the other hand, configurations that repeatedly swap their rankings perform similarly well and the performance difference in the current epoch or rung is simply due to noise. We want to measure this noise and use it to automatically estimate the threshold value $\epsilon$ to be used in the soft-ranking described above.

Formally we can define a set of pairs of configurations that perform similarly well by the following:
\begin{equation}
\begin{split}
S: \{ (c, c^\prime): & \left(\pi_{r_j}(c) > \pi_{r_j}(c^\prime) \land \pi_{r_k}(c) < \pi_{r_k}(c^\prime) \land \pi_{r_l}(c) > \pi_{r_l}(c^\prime)\right) \\ & \lor \left(\pi_{r_j}(c) < \pi_{r_j}(c^\prime) \land \pi_{r_k}(c) > \pi_{r_k}(c^\prime) \land \pi_{r_l}(c) < \pi_{r_l}(c^\prime)\right) \},
\end{split}
\end{equation}

for resource levels (e.g. epochs -- not rungs) $r_j > r_k > r_l$, using the same notation as earlier to refer to resources. In practice we have per-epoch validation performance statistics and use these to find resource levels $r_j, r_k, r_l$ that have configurations with the criss-crossing behaviour (there can be several epochs between such resource levels). We only consider configurations $(c, c^\prime)$ that made it to the latest rung, so $r\eta^{K_t-1} \geq r_j > r\eta^{K_t-2}$. However, we allow for the criss-crossing to happen across epochs from any rungs.
The value of $\epsilon$ can then be calculated as the $N$-th percentile of distances between the performances of configurations in $S$:
$$\epsilon=\text{P}_{N, (c, c^\prime) \in S}|f_{r_j}(c)-f_{r_j}(c^\prime)|.$$

The exact value of $r_j$ depends on the considered pair of configurations $(c, c^\prime)$. To uniquely define $f_{r_j}$, we take the maximum resources $r_j$ currently available for both configurations in the considered pair $(c, c^\prime)$. Let us consider the following example setup: the top rung has 8 epochs and the next one has 4 epochs, there are three configurations $c_a, c_b, c_c$ that made it to the top rung and were trained for 8, 8 and 6 epochs so far respectively. Assuming there was criss-crossing within each pair $(c_a, c_b)$, $(c_a, c_c)$ and $(c_b, c_c)$, the set of distances between configurations in $S$ is $\left\{|f_8(c_a)-f_8(c_b)|, |f_6(c_a)-f_6(c_c)|, |f_6(c_b)-f_6(c_c)|\right\}$. The value of $\epsilon$ is recalculated every time we receive new information about the performances of configurations. Initially the value of $\epsilon$ is set to 0, which means that we check for exact ranking if we cannot yet calculate the value of $\epsilon$.

==> arXiv v2 PASHA/related.tex <==
Real-world machine learning systems often rely on a large number of hyperparameters and require testing many combinations to identify suitable values. This makes data-inefficient techniques such as Grid Search or Random Search \citep{Bergstra2012RandomOptimization} very expensive in most practical scenarios.
Various approaches have been proposed to find good parameters more quickly, and they can be classified into two main families:  
1) Bayesian Optimization: evaluates the most promising configurations by modelling their performance. The methods are sample-efficient but often designed for environments with limited amount of parallelism; 2) Multi-fidelity: sequentially allocates more resources to configurations with better performance and allows high level of parallelism during the tuning. Multi-fidelity methods have typically been faster when run at scale and will be the focus of this work.
Ideas from these two families can also be combined together, for example as done in BOHB by \citet{Falkner2018BOHB:Scale}, and we will test a similar method in our experiments.

Successive Halving (SH) \citep{karnin2013almost, jamieson2016non} is conceptually 
the simplest multi-fidelity method. Its key idea is to run all configurations using a small amount of resources and then successively promote only a fraction of the most promising configurations to be trained using more resources. Another popular multi-fidelity method, called Hyperband \citep{hyperband}, performs SH with different early schedules and number of candidate configurations. ASHA \citep{li2020asha} extends the simple and very efficient idea of successive halving by introducing 
asynchronous evaluation of different configurations, which leads to further practical speedups thanks to better utilisation of workers in a parallel setting.

Related to the problem of efficiency in HPO, cost-aware HPO explicitly accounts for the cost of the evaluations of different configurations.
Previous work on cost-aware HPO for multi-fidelity algorithms such as CAHB~\citep{ivkin2021cost} keeps a tight control on the budget spent during the HPO process. This is different from our work, as we reduce the budget spent by terminating the HPO procedure early instead of allocating the compute budget in its entirety. Moreover, PASHA could be combined with CAHB to leverage the cost-based resources allocation.

Recently, researchers considered dataset subsampling to speedup HPO and NAS. \citet{shim2021coreset} have combined coresets with PC-DARTS \citep{Xu2020PC-DARTS:Search} and showed that they can find  well-performing architectures using only 10\% of the data and 8.8x less search time. Similarly, \citet{visalpara2021adata} have combined subset selection methods with the Tree-structured Parzen Estimator (TPE) for HPO \citep{bergstra2011TPE}. With a 5\% subset they obtained between an 8x to 10x speedup compared to standard TPE. However, in both cases it is difficult to say in advance what subsampling ratio to use. For example, the 10\% ratio in \citep{shim2021coreset} incurs no decrease in accuracy, while reducing further to 2\% leads to a substantial (2.6\%) drop in accuracy.
In practice, it is difficult to find a trade-off between the time required for tuning (proportional to the subset size) and the loss of performance for the final model because these change, sometimes wildly, between datasets.
Further, \citet{Zhou2020EcoNAS:Search} have observed that for a fixed number of iterations, rank consistency is better if we use more training samples and fewer epochs rather than fewer training samples and more epochs. This observation gives further motivation for using the whole dataset for HPO/NAS and design new approaches, like PASHA, to save computational resources.


==> arXiv v2 PASHA/setup.tex <==
\label{sec:setup}
The problem of selecting the best configuration of a machine learning algorithm to be trained is formalized in \citep{jamieson2016non} 
as a non-stochastic bandit problem. In this setting the learner (the hyperparameter optimizer)
receives $N$ 
hyperparameter configurations and it has to identify the best performing one with the
constraint of not spending more than a fixed amount of resources $R$ (e.g. total number of training epochs) on a specific configuration.
$R$ is considered given, but in practice users do not have a good 
way for selecting it, 
which can have undesirable consequences: if the value is too small, the model performance will be sub-optimal, while if the budget is too large, the user will incur a significant cost without any practical return. This leads users to overestimate $R$, setting it to a large amount of resources in order to guarantee the convergence of the model. We maintain the concept of maximum amount of resources in our algorithm but we prefer to interpret $R$ as a ``safety net'', a cost not to be surpassed (e.g. in case an error prevents a normal behaviour of the algorithm), instead of the exact amount of resources spent for the optimization.

This setting could be extended with additional assumptions, based on empirical observation, removing some extreme cases and leading to a more practical setup.
In particular, when working with large datasets we observe that the curve of the loss for configurations (called arms in the bandit literature)
continuously decreases (in expectation). Moreover, 
``crossing points'' between the curves are rare (excluding noise), and they are almost always in the very initial part
of the training procedure.
\citet{Viering2021TheReview, Mohr2022LearningSurvey} provide an analysis of learning curves and note that in practice most learning curves are well-behaved, with \citet{bornschein2020small, Domhan2015SpeedingCurves} reporting similar findings.

More formally, let us define $R$ as the maximum number of resources needed to train an ML algorithm to convergence. Given $\pi_m(i)$ the ranking of configuration $i$ after using $m$ resources for training, there exists minimum $\RS$ much smaller than $R$ such that for all amounts of resources $r$ larger than $\RS$ the rankings of configurations trained with $r$ resources remain the same: $\exists \RS \ll R : \forall i \in \{\text{configurations}\}, \forall r > \RS, \pi_{\RS}(i) = \pi_r(i)$.
The existence of such a quantity, limited to the best performing configuration, is also assumed by \citet{jamieson2016non}, and it is leveraged to quantify the budget required to identify the best performing configuration. If we knew $\RS$, it would be sufficient to run all configurations with exactly that amount of resources to identify the 
best one and then just train the model from scratch with all the data using that configuration.
Unfortunately that quantity is unknown and can only be estimated during the optimization procedure. Note that in practice there is noise involved in training of neural networks, so similarly performing configurations will repeatedly swap their ranks.

